MIA-Bench: Towards Better Instruction Following Evaluation of Multimodal LLMs

We introduce MIA-Bench, a new benchmark designed to evaluate multimodal large language models (MLLMs) on their ability to strictly adhere to complex instructions. Our benchmark comprises a diverse set of 400 image-prompt pairs, each crafted to challenge the models' compliance with layered instructions in generating accurate responses that satisfy specific requested patterns. Evaluation results from a wide array of state-of-the-art MLLMs reveal significant variations in performance, highlighting areas for improvement in instruction fidelity. Additionally, we create extra training data and explore supervised fine-tuning to enhance the models' ability to strictly follow instructions without compromising performance on other tasks. We hope this benchmark not only serves as a tool for measuring MLLM adherence to instructions, but also guides future developments in MLLM training methods.

==> sections/7.checklist.tex <==
\clearpage
\section*{Checklist}


\begin{enumerate}

\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \answerYes{}
  \item Did you describe the limitations of your work?
    \answerYes{}
  \item Did you discuss any potential negative societal impacts of your work?
    \answerNA{}
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    \answerYes{}
\end{enumerate}

\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
     \answerNA{}
	\item Did you include complete proofs of all theoretical results?
     \answerNA{}
\end{enumerate}

\item If you ran experiments (e.g. for benchmarks)...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    \answerYes{Benchmark data and evaluation code: \url{https://anonymous.4open.science/r/MIA-Bench-FC72}} 
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
    \answerYes{}
	\item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    \answerYes{We mentioned in Section 3.}
	\item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
    \answerNA{}
\end{enumerate}

\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
    \answerYes{}
  \item Did you mention the license of the assets?
    \answerNo{}
  \item Did you include any new assets either in the supplemental material or as a URL?
    \answerYes{Benchmark and evaluation code: \url{https://drive.google.com/drive/folders/19_xU6rqpU4BYHIeo4AVCydAJ20V9yQ-7?usp=sharing}} 
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    \answerNA{} The image sources are from public datasets widely used in academia.
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
    \answerNA{}
\end{enumerate}

\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
    \answerYes{} In section we described how we (the authors) manually constructed the benchmark.
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
    \answerNA{}
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
    \answerNA{}
\end{enumerate}

\end{enumerate}

==> tables/RL-compare.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
\begin{table}[]
\centering
\huge
\renewcommand{\arraystretch}{1.5} % Adjust the factor to increase or decrease row height
\resizebox{\columnwidth}{!}{%
\begin{tabular}{cccccccccc}
\hline
  \textbf{Model} & \textbf{Total Score} & \textbf{Describe} & \textbf{Length Limit} & \textbf{Linguistics} & \textbf{Grammar} & \textbf{Mention} & \textbf{Math} & \textbf{Perspective} & \textbf{OCR}\\ % 


\rowcolor[HTML]{EFEFEF}LLaVA-1.6-13b-vicuna\citep{liu2023improved} & 69.16&	86.75&	69.88&	82.07	&64.77	&74.99	&48.56&	77.50&	75.83 \\ %\hline
LLaVA-1.6-13b ckpt25* & 68.30 & 85.71 & 70.71 & 82.15 & 70.49 & 70.79 & 58.61 & 65.00  & 81.71\\ 
\rowcolor[HTML]{EFEFEF}LLaVA-1.6-13b ckpt500* & 63.60 & 87.16 & 53.32 & 83.17 & 63.13 & 75.03 & 61.42 & 85.19 & 83.13 \\ \hline
\end{tabular}%
}
\caption{Evaluation result before and after(denoted by *) RL on diverse instruction data on MIA-Bench.}
\label{tab:Evaluation result of MLLMs before and after RL}
\end{table}



==> tables/claude_and_gpt4v.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
\begin{table}[]
\centering
\resizebox{\columnwidth}{!}{%
\begin{tabular}{ccccccc}
\hline
  \textbf{Model} & \textbf{Total Score} & \textbf{Describe} & \textbf{Length Limit} & \textbf{Linguistics} & \textbf{Grammar} & \textbf{Mention} \\ % 
  %\hline

\rowcolor[HTML]{EFEFEF}claude-3-sonnet_{20240229}\citep{claude2022}  & 96.50 & 96.86  & 94.64 & 98.04 & 99.59 & 95.33  \\ %\hline
gpt-4-vision-preview\citep{openai2024gpt4} & 97.29 & 97.62  & 94.23 & 100.00 & 98.45 & 97.89\\ \hline

\end{tabular}%
}
\caption{Evaluation result of Claude-3 and GPT-4V by Claude-3.}
\label{tab:Evaluation result of MLLMs by claude 3}
\end{table}

==> tables/complexity_statistics.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
\begin{table}[]
\centering
\resizebox{\columnwidth}{!}{%
\begin{tabular}{|l|r|r|r|r|r|}
\hline
\textbf{Image Source} &
  \multicolumn{1}{l|}{\textbf{basic}} &
  \multicolumn{1}{l|}{\textbf{intermediate}} &
  \multicolumn{1}{l|}{\textbf{advanced}} &
  \multicolumn{1}{l|}{\textbf{creative}} &
  \multicolumn{1}{l|}{\textbf{complex}} \\ \hline
COCO    & 9  & 15  & 14 & 18 & 24 \\ \hline
SBU     & 13 & 31  & 13 & 5  & 18 \\ \hline
Flickr  & 10 & 28  & 18 & 7  & 17 \\ \hline
Textvqa & 9  & 45  & 9  & 14 & 3  \\ \hline
Total   & 41 & 119 & 54 & 44 & 62 \\ \hline
\end{tabular}%
}
\caption{Statistics of overall instruction complexity distribution.}
\label{tab:statistics of overall instruction complexity distribution}
\end{table}

==> tables/instruction_type_statistics.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
\begin{table}[]
\centering
\resizebox{\columnwidth}{!}{%
\begin{tabular}{|l|r|r|r|r|r|}
\hline
\textbf{Image Source} &
  \multicolumn{1}{l|}{\textbf{describe}} &
  \multicolumn{1}{l|}{\textbf{length\_limit}} &
  \multicolumn{1}{l|}{\textbf{mention}} &
  \multicolumn{1}{l|}{\textbf{linguistics}} &
  \multicolumn{1}{l|}{\textbf{grammar}} \\ \hline
COCO    & 77  & 59  & 44  & 37  & 13 \\ \hline
SBU     & 78  & 46  & 52  & 25  & 18 \\ \hline
Flickr  & 78  & 43  & 47  & 28  & 13 \\ \hline
TextVQA & 75  & 38  & 50  & 22  & 11 \\ \hline
Total   & 308 & 186 & 193 & 112 & 55 \\ \hline
\end{tabular}%
}
\caption{Statistics of overall instruction categories distribution.}
\label{tab:statistics of overall instruction categories distribution}
\end{table}

==> tables/preference_data_coco.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
% \usepackage[table,xcdraw]{xcolor}
% Beamer presentation requires \usepackage{colortbl} instead of \usepackage[table,xcdraw]{xcolor}
\begin{table}[h]
\centering
\renewcommand{\arraystretch}{1.6} % Adjust the factor to increase or decrease row height
\resizebox{\columnwidth}{!}{%
\begin{tabular}{ccccccc}
\hline
\textbf{} & \textbf{Total Score} & \textbf{Describe} & \textbf{Length Limit} & \textbf{Linguistics} & \textbf{Grammar} & \textbf{Mention} \\ %\hline
\rowcolor[HTML]{EFEFEF}GPT-4V             & 91.44               & 94.60            & 92.25                & 99.44               & 91.67           & 91.67           \\ %\hline
 
GPT-4V-worse       & 73.03               & 89.89            & 86.53                & 91.94               & 65.38           & 75.21           \\ \hline
\end{tabular}%
}
\caption{Response quality of the GPT-4V generated preference data.}
\label{tab:preference-data-coco}
\end{table}
